Bringing freedom in variable choice when searching counter-examples in floating point programs

Program verification techniques typically focus on finding counter-examples that violate properties of a program. Constraint programming offers a convenient way to verify programs by modeling their state transformations and specifying searches that seek counter-examples. Floating-point computations present additional challenges for verification given the semantic subtleties of floating point arithmetic. % This paper focuses on search strategies for CSPs using floating point numbers constraint systems and dedicated to program verification. It introduces a new search heuristic based on the global number of occurrences that outperforms state-of-the-art strategies. More importantly, it demonstrates that a new technique that only branches on input variables of the verified program improve performance. It composes with a diversification technique that prevents the selection of the same variable within a fixed horizon further improving performances and reduces disparities between various variable choice heuristics. The result is a robust methodology that can tailor the search strategy according to the sought properties of the counter example.

==> makeplot <==
# Scale font and line width (dpi) by changing the size! It will always display stretched.

set xlabel 'Strategy'
set ylabel 'Time(s)'
set title 'Impact of each feature'
set xtics rotate # rotate labels on the x axis
set key inside top  right

plot '<(tail -n 8 "data.txt")' using 0:xtic(1)

#plot for [col=2:5] 'data.txt' using 0:col with lines title columnheader\
					, '<(tail -n 8 "data.txt")' using 0:xtic(1)
#set term png   
#set output "out.png"
